A first-principles study of bilayer 1T'-WTe2/CrI3: A candidate topological spin filter

The ability to manipulate electronic spin channels in 2D materials is crucial for realizing next-generation spintronics. Spin filters are spintronic components that polarize spins using external fields or material properties like magnetism. Recently, topological protection from backscattering has emerged as an enticing feature through which to enhance the robustness of 2D spin filters. In this work, we propose and then characterize one of the first 2D topological spin filters: bilayer CrI3/1T'-WTe2 (BLCW). To do so, we use a combination of DFT, maximally localized Wannier functions, and quantum transport simulations to demonstrate that the BLCW satisfies the principal criteria for being a topological spin filter; namely that it is gapless, exhibits spin-polarized charge transfer (SPCT) from WTe2 to CrI3 that renders the BLCW metallic, and has a topological boundary which retains the edge conductance of monolayer (ML) 1T'-WTe2. We observe that the atomic magnetic moments on Cr from DFT are approximately 3.2 mB/Cr in the BL compared to 2.9 mB/Cr with small negative ferromagnetic (FM) moments induced on the W atoms in freestanding ML CrI3. Subtracting the charge/spin densities of the constituent ML's from those of the BLCW further reveals SOC-enhanced SPCT from WTe2 to CrI3. We find that the BLCW is topologically trivial by showing that its Chern number is zero. Lastly, we show that interfacial scattering at the boundary between the terraced materials does not remove WTe2's edge conductance. This evidence indicates that BLCW is gapless, magnetic, and topologically trivial, meaning that a terraced WTe2/CrI3 BL heterostructure in which only a portion of a WTe2 ML is topped with CrI3 is a promising candidate for a 2D topological spin filter. Our results further suggest that 1D chiral edge states may be realized by stacking FM ML's, like CrI3, atop 2D nonmagnetic Weyl semimetals like 1T'-WTe2.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx.tex <==


